Efficient Planning in Combinatorial Action Spaces with Applications to Cooperative Multi-Agent Reinforcement Learning

A practical challenge in reinforcement learning are combinatorial action spaces that make planning computationally demanding. For example, in cooperative multi-agent reinforcement learning, a potentially large number of agents jointly optimize a global reward function, which leads to a combinatorial blow-up in the action space by the number of agents. As a minimal requirement, we assume access to an argmax oracle that allows to efficiently compute the greedy policy for any Q-function in the model class. Building on recent work in planning with local access to a simulator and linear function approximation, we propose efficient algorithms for this setting that lead to polynomial compute and query complexity in all relevant problem parameters. For the special case where the feature decomposition is additive, we further improve the bounds and extend the results to the kernelized setting with an efficient algorithm.

==> parts/experiments.tex <==

\section{Experiments} \label{sec:experiments}
In this section we present experiments on a cooperative multi-agent cliff-walking experiment.
We results contain algorithms: MCLSPI-EGSS, MCLSPI-DAV, Politex-EGSS, Politex-DAV

==> parts/extensions.tex <==
\section{Extensions}\todoj{put this here for now but this can potentially go elsewhere}
\subsection{Argmax Oracle}


\subsection{Kernelized Algorithm}
Add all the new notation for kernel setting and state the theorem.
    Kernel proofs are in Appendix \ref{app:kernel setting} \todoj{if we keep it we just refer to the appendix}

==> parts/theory.tex <==


\section{Theoretical Results} \label{sec:theoretical results}\todoj{results from this section get distributed into section 4/5, then remove this section}
In this section we provide a theorem for each of the four variants of the main algorithm, as discussed in the previous section. 
The theorems provide bounds on the computation and query complexity of the main algorithm, and the sub-optimality of the output policy's value function.
The complete proofs of all the results can be found in \cref{app: theorem proofs}.

\begin{theorem}[MA-MC-LSPI Sub-Optimality] \label{thm:ma-mc-lspi sub-optimality}
    With $z=2m-1$ when \textsc{Uncertainty Check with DAV} is used, and $z = \sqrt{d}$ when \textsc{Uncertainty Check with EGSS} is used.
    If \cref{ass: feature decomposition} holds and $\epsilon \neq 0$, then with probability at least $1 - \delta$, the policy $\pi_{K-1}$, output by \textsc{Confident Multi-Agent MC-LSPI} satisfies
    \begin{equation*}
        V^*(\rho) - V_{\pi_{K-1}}(\rho) \leq \frac{64 \epsilon \sqrt{d} z}{(1-\gamma)^2} (1 +\log(1+m b^2 \epsilon^{-2} d^{-1}))^{1/2}.
    \end{equation*}
    Further on, the query cost is $\cO\left(\tfrac{d^2}{\epsilon^2 (1-\gamma)^4} \right)$
    and computation cost is $\poly(d, \frac{1}{1 - \gamma}, \frac{1}{\kappa}, \log(\frac{1}{\delta}), \log(b), m, A)$.
    
    While if $\epsilon = 0$, then for any $\kappa > 0$, with probability at least $1 - \delta$, the policy $\pi_{K-1}$, output by \textsc{Confident Multi-Agent MC-LSPI} satisfies
    \begin{equation*}
        V^*(\rho) - V_{\pi_{K-1}}(\rho) \leq \kappa. 
    \end{equation*}
    Further, the query cost is $\cO\left(\tfrac{z^2 d^3}{\kappa^2 (1-\gamma)^8} \right)$
    and computation cost is $\poly(d, \frac{1}{1 - \gamma}, \frac{1}{\kappa}, \log(\frac{1}{\delta}), \log(b), m, A)$.
    With parameters settings for both cases above as defined in \cref{app: theorem proofs}.
    Moreover, the above results also hold under \cref{ass: argmax oracle} when \textsc{Uncertainty Check with EGSS} is used.
\end{theorem}

\begin{theorem}[MA-MC-Politex Sub-Optimality] \label{thm:ma-mc-politex sub-optimality}
    With $z=2m-1$ when \textsc{Uncertainty Check with DAV} is used, and $z = \sqrt{d}$ when \textsc{Uncertainty Check with EGSS} is used.
    If \cref{ass: feature decomposition} holds and $\epsilon \neq 0$, then with probability at least $1 - \delta$, the policy $\bar \pi_{K-1}$, output by \textsc{Confident Multi-Agent MC-Politex} satisfies
    \begin{equation*}
        V^*(\rho) - V_{\pi_{K-1}}(\rho) \leq \frac{32 \epsilon \sqrt{d} z}{1-\gamma} (1 +\log(m b^2 \epsilon^{-2} d^{-1}))^{1/2}.
    \end{equation*}
    Further, the query cost is $\cO\left(\tfrac{md}{\epsilon^4 (1-\gamma)^5} \right)$
    and computation cost is $\poly(d, \frac{1}{1 - \gamma}, \frac{1}{\kappa}, \log(\frac{1}{\delta}), \log(b), m, A)$.
    
    While if $\epsilon = 0$, then for any $\kappa > 0$, with probability at least $1 - \delta$, the policy $\bar \pi_{K-1}$, output by \textsc{Confident Multi-Agent MC-Politex} satisfies
    \begin{equation*}
        V^*(\rho) - V_{\pi_{K-1}}(\rho) \leq \kappa. 
    \end{equation*}
    Further on, the query cost is $\cO\left(\tfrac{mz^2 d^3}{\kappa^4 (1-\gamma)^9} \right)$
    and computation cost is $\poly(d, \frac{1}{1 - \gamma}, \frac{1}{\kappa}, \log(\frac{1}{\delta}), \log(b), m, A)$.
    With parameters settings for both cases above as defined in \cref{app: theorem proofs}.
\end{theorem}
